Deep Learning of Sea Surface Temperature Patterns to Identify Ocean Extremes

We perform an out-of-distribution analysis of ~12,000,000 semi-independent 128x128 pixel^2 SST regions, which we define as cutouts, from all nighttime granules in the MODIS R2019 Level-2 public dataset to discover the most complex or extreme phenomena at the ocean surface. Our algorithm (Ulmo) is a probabilistic autoencoder, which combines two deep learning modules: (1) an autoencoder, trained on ~150,000 random cutouts from 2010, to represent any input cutout with a 512-dimensional latent vector akin to a (non-linear) EOF analysis; and (2) a normalizing flow, which maps the autoencoder's latent space distribution onto an isotropic Gaussian manifold. From the latter, we calculate a log-likelihood value for each cutout and define outlier cutouts to be those in the lowest 0.1% of the distribution. These exhibit large gradients and patterns characteristic of a highly dynamic ocean surface, and many are located within larger complexes whose unique dynamics warrant future analysis. Without guidance, Ulmo consistently locates the outliers where the major western boundary currents separate from the continental margin. Buoyed by these results, we begin the process of exploring the fundamental patterns learned by Ulmo, identifying several compelling examples. Future work may find that algorithms like Ulmo hold significant potential/promise to learn and derive other, not-yet-identified behaviors in the ocean from the many archives of satellite-derived SST fields. As important, we see no impediment to applying them to other large, remote-sensing datasets for ocean science (e.g., sea surface height, ocean color).

==> acronym/CHANGES <==
Version 1.47 (Apr 2020)

- Fixed \Iac macro expansion bug
-- Tobias Oetiker
- Fixed regression in commands for capitalisation
-- Marcus Meeßen
- Fixed bug were output depends on the position of the list of acronyms
-- Marcus Meeßen
- Fixed \Iac hyperlink nesting
-- Marcus Meeßen

Version 1.46 (Mar 2020)

- Fix merge error

Version 1.45 (Mar 2020)

-  Fixed hyperref regression and the longstanding "missing aux" bug.
-- Marcus Meeßen
 
Version 1.44 (Feb 2020)

- added the |printonlyreused| option, which allows to automatically exclude acronyms from the list of acronyms if they are used only once
-- Marcus Meeßen

Version 1.43 (Feb 2020)

fixed unconventional dots spacing in list of acronyms
-- Marcus Meeßen

enhanced list of acronyms with hyperrefs
-- Marcus Meeßen

fixed collisions between acronyms and package commands, can be turned of with
the |noacroprefix| option
-- Marcus Meeßen

Version 1.42 (Nov 2019)

fix the carriage return with long lines (line 234/235) -- Philippe Chauvat

fix page number display for acfi Acfi -- Tobi Oetiker

fix double space and missing used flag with acfi -- Horst Schirmeier

two features were added -- Oz Davidi
 * Now it is possible to forbid a line break between the full name and the short name (when they are printed together). It is possible to control it individually (for each command), and also globally (with the |nolinebreak| option).
 * Added the \Ac{p,f,fp,l,lp,lu} commands. They work exactly the same way as the \ac commands, but prints the full name, starting with an upper case letter (in case it was defined with a lower case letter).

correting issue with long lines due to carriage return misplaced -- Philippe Chauvat 

Version 1.41 (Mar 2015)

change names of internal macros to avoid nameing conflics with pageslts
package -- Tobi Oetiker and Jason Mills

Version 1.40 (Sept 2014)

remove \hskip\z@ instances, since they cause bad formating
since space at the end of a line can not be collapsed anymore
-- Hartmut Henkel

Version 1.39 (Aug 2014)

make the appearance of labels consistent whether or not the acronym environment
has its optional argument provided
-- Yann Leprince

Version 1.38 (Oct 2012)

add support for dynamic indefinite articles depending on the acronym form used
-- Ash Hughes 

fix for non hyphenation of first word in long form
-- Martin Rüßler

fix description of acrodefplural
-- Joel Johnson

\ac* should NOT set the used flag ... now it does not
-- Martin Falk

Version 1.36 (Sept 2010) Uwe Bieling disable hyperlinks in nolist mode.
Tobi added mbox to prevent hyphenation of short form of acronyms.

Version 1.35 (Oct 2009) Added support for nonstandard plural forms.
Changed management of default short form in acronym definition.
Now, one can safely use \newacro in the preamble to define acronyms.
-- Sergio Callegari

Version 1.34 (Jan 2009) Make sure the s in acp gets smaller as well when the
smaller package option is used.
-- Tobi Oetiker

Version 1.33 (Dec 2008) Make the alternate acronym environment
representation work. The test for the presence of optional argument was
rather broken. When it worked, it did so for all the wrong reasons
-- Enrico Gregorio

Version 1.32 (May 2008) Altered code to redefine labels in
order to cope with unreproducable bug-reports. Warnings turned into infos.
-- Ulrich Diez

Version 1.31 (April 2008) Renamed clearlist to AC@clearlist to fix
name conflict with jurabib
-- Philipp Lehman

Version 1.30 (April 2008) Corrected code to redefine labels and
adjusted behavior with \cmd{\AC@used}.
-- Ulrich Diez

Version 1.29 (April 2008) let withpage option show the 'corect' page number
and not just the first one.
-- Domagoj Babic (babic in cs.ubc.ca) (with help from Ulrich Diaz)

Version 1.28 (April 2008) fixed layout of addpage list
-- Tobias Oetiker (tobi with oetiker.ch)

Version 1.27 (April 2008) add option 'addpage' to add pagenumber of first
occurenace to list of acronyms.
-- Tobias Oetiker (tobi with oetiker.ch)

Version 1.26 (June 2006) supress lone item when nolist is in effect
-- Immo Köster <Immo.Koester there rwth-aachen.de>

Version 1.25 (November 2005) properly handle acronyms in pdfbookmarks
-- Heiko Oberdiek <oberdiek there uni-freiburg.de>

Version 1.24 (October 2005) ac* commands are now not fragile anymore ... 
-- José Emilio Vila Forcén jose.vila there cui.unige.ch

Version 1.23 (October 2005) fixed typo in nolist option. added comment about fragility of ac commands.
-- Tobias Oetiker (tobi with oetiker.ch)

Version 1.22 (October 2005) added starred versions of ac(p), acf(p), acs(p),
acl(p), acfi, acsu & aclu 
-- Stefan Pinnow (Mo-Gul here gmx.net)

Version 1.21 (September 2005): fixed the  \acused command again ... broke it
in 1.20 (this time I amended the docs, so that the intention becomes clear).
Set acronyms as used in the first run, not only in the second one.
-- Tobi Oetiker tobi at oetiker.ch

added new option nolist to suppress printing the acronym list all together
-- José Emilio Vila Forcén jose.vila there cui.unige.ch

Version 1.20 (August 2005): make the acused command actually work
-- Richard Walker Richard.Walker there cs.anu.edu.au

Version 1.19 (April 2005): three new commands acused (set-used), acsu (adds to used), aclu (adds to used)
--  Lee Netherton ltn100 there ohm.york.ac.uk

Version 1.18 (April 2005): added additional format option for Full Name (acfi)
--  Manuel G"ortz mgoertz there kom.tu-darmstadt.de

Version 1.17 (November 2004): added don't use acronyms (dua) option
--  Oliver Creighton

Version 1.16 (November 2004): fix version number
-- Oliver Creighton <creighto there in.tum.de>
new option to suppress all acronym printing -- don't use acronyms (dua)

Version 1.16 (November 2004): fix version number
-- tobi there oetiker.ch

Version 1.15 (November 2004): fix for acresetall to work when ac is called
in grouped material.
-- Hendri Adriaens <Hendri there uvt.nl>

Version 1.14 (October 2004): fix acsp and acfp for footnote mode
-- Markus Ortner <m.ortner there icie.jku.at>

Version 1.13 (July 2004): deflist renamed to AC there deflist to
avoid unnecessary naming conflict.
--  Peter May <peter.may there philips.com>

Version 1.13 (July 2004): printonlyused was not working anymore
--  Tobi Oetiker <tobi at oetiker.ch>

Version 1.13 (July 2004): if the footnote option was on, footnotes were
printed for ALL acronyms ALL the time, this looked rather odd if the same
acronym was used more than once on the same page. Changed it so that
footnote printing follows the same rules as normal acronym printing (only
print footnote first time). One might think about changing this, so that
either footnotes get printed 'once' per page. Or that the footnote marks are
issued once per acronym and page, so that all instances of the same acronym
on a page get the same footnote mark. Feel free to contribute patches.
--  Tobi Oetiker <tobi at oetiker.ch>

Version 1.12 (June 2004): Make acronyms robust and compatible
with pdf bookmarks.
--  Danie Els <dnjels there sun.ac.za>

Version 1.11 (June 2004): Make hyperlinks work inside optional
item text by replacing hypertarget with raisedhypertarget
--  Martin Salois <Martin.Salois there drdc-rddc.gc.ca>

Version 1.10 (May 2004): Fix for the bug of a \cs{}\cs{} following an
acronym. Add footnote optional out for \cmd{\acs}. Fix for list of acronyms
in front matter and addition of \cmd{\acroextra} command.
-- Danie Els <dnjels there sun.ac.za>

Version 1.9 (October 2003): Fix hyperref processing to work regardles 
of calling order. 'printused' now prints every acronym used not only 
the ones called through \ac.
-- Danie Els <dnjels there sun.ac.za> and Tobi Oetiker

Version 1.8 (October 2003): When the hyperref package is loaded before the
acronym package, all acronyms will become a hyperlink to their own
definition.
-- Martin Salois <Martin.Salois there drdc-rddc.gc.ca>

Version 1.7 (September 2003): Added \acresetall for resetting the 'used'-tag
of \ac. With the new option 'printonlyused', the acronym-list will consist of 
the used acronyms only and not of all defined acronyms; Optional in a special 
deflist - environment.
-- Sebastian Max <smx there comnets.rwth-aachen.de>

Version 1.6 (May 2000): Added the smaller option and the macros \acsfont, 
\acffont, and \acfsfont used to control the appearance of  \acs and \acf.
-- Ingo Lepper <lepper there math.uni-muenster.de>

Version 1.5 (May 2000): Added support for english plural forms and the
footnote option.
-- David Sterratt <David.C.Sterratt there ed.ac.uk>

Version 1.4 (February 2000): A formatted acronym string, which is allowed
to contain indices, for example, is now possible. For this purpose
the syntax of \acro and \acrodef now permits an optional argument:
  \acro{<acronym>}{<full name>}                 (without opt. arg.)
  \acro{<acronym>}[<short name>]{<full name>}   (with opt. arg.)
The user macros \ac, \acs, \acl, and \acf print now <short name>
instead of <acronym>, if available.
-- Heiko Oberdiek <oberdiek there ruf.uni-freiburg.de>

Version 1.2 (August 1996) features a new command: \acl to print the
expanded acronym with out even mentioning that there is an acronym for
this word.
-- Tobias Oetiker <tobi at oetiker.ch>

